Advancing Fairness in Natural Language Processing: From Traditional Methods to Explainability

The burgeoning field of Natural Language Processing (NLP) stands at a critical juncture where the integration of fairness within its frameworks has become an imperative. This PhD thesis addresses the need for equity and transparency in NLP systems, recognizing that fairness in NLP is not merely a technical challenge but a moral and ethical necessity, requiring a rigorous examination of how these technologies interact with and impact diverse human populations. Through this lens, this thesis undertakes a thorough investigation into the development of equitable NLP methodologies and the evaluation of biases that prevail in current systems. First, it introduces an innovative algorithm to mitigate biases in multi-class classifiers, tailored for high-risk NLP applications, surpassing traditional methods in both bias mitigation and prediction accuracy. Then, an analysis of the Bios dataset reveals the impact of dataset size on discriminatory biases and the limitations of standard fairness metrics. This awareness has led to explorations in the field of explainable AI, aiming for a more complete understanding of biases where traditional metrics are limited. Consequently, the thesis presents COCKATIEL, a model-agnostic explainability method that identifies and ranks concepts in Transformer models, outperforming previous approaches in sentiment analysis tasks. Finally, the thesis contributes to bridging the gap between fairness and explainability by introducing TaCo, a novel method to neutralize bias in Transformer model embeddings. In conclusion, this thesis constitutes a significant interdisciplinary endeavor that intertwines explicability and fairness to challenge and reshape current NLP paradigms. The methodologies and critiques presented contribute to the ongoing discourse on fairness in machine learning, offering actionable solutions for more equitable and responsible AI systems.

==> OLD_SOTA.tex <==
\chapter{Fairness and Explainability, State of the Art}\label{SOTAOLD}

In the rapidly advancing field of NLP, the balance between technical innovation and ethical responsibility is crucial. This chapter, building on the introductory discussion of fairness's ethical and legal aspects, delves into the latest methodologies in NLP aimed at addressing these concerns.

Here, we explore a range of strategies for mitigating bias, from initial data preparation to algorithm adjustments and final evaluations, presenting a comprehensive view of efforts to enhance fairness in NLP. We then transition to the concept of explainability in NLP, highlighting how making complex language models transparent can build trust and accountability.

The discussion culminates with an examination of concept-based approaches in Explainable AI (XAI), focusing on understanding model-driven concepts and their role in creating more interpretable and equitable AI systems. This chapter aims to present a clear and concise overview of the state-of-the-art in NLP.


\section{Bias mitigation techniques}
%Having extensively explored the technical intricacies of transformer models, which form the foundation of contemporary Natural Language Processing applications, it becomes imperative to scrutinize the broader implications of their application. As these models gain ubiquity, questions of fairness, bias, and representativeness inevitably emerge.


Bias in NLP systems has received a significant attention in recent years, with researchers and practitioners exploring various methods for mitigating bias in NLP models. The mitigation of bias in NLP can be approached through various strategies, including \textit{pre-processing}, \textit{in-processing}, and \textit{post-processing} methods. Each of these strategies offers different advantages and limitations in addressing bias.


%preprocessing
\paragraph{Pre-processing methods}
The first approach to mitigate bias is to apply \emph{pre-processing} techniques to the data used to train the model. This method focuses on modifying the training data before the model learns from it, leading to more generalized and fairer models. Researchers like \cite{lu2020gender} highlight the advantages of this approach, emphasizing its capacity to tackle bias at its root. By altering the training data, the models developed are less likely to inherit biases, thereby promoting fairness and generalization.

We can reduce the bias directly in the text of the training dataset. For example, in the case of gender bias like the study in this paper, the most classic technique is to remove explicit gender indicators \citep{de2019bias}. This technique is the one we will use to compare our proposed strategy to another one commonly used in industry. This technique is indeed simple to implement and makes it possible to reduce the bias, but in a partial and not very localized manner. %{\color {magenta} maybe say a bit more here.  What about bias reduction vs. accuracy tradeoff?} {\color{blue} Je ne suis pas sur de comment mettre ça ici. Ce n'est pas que les méthodes pre-processing qui ont ce soucis mais un peu tout type de méthode de réduction de biais classique. De plus on a une partie sur ces problematiques en section 2.2. Est ce que ça ne ferait pas doublon?}
Other classical techniques can be used, like identifying biased data in word embeddings, which represent words in a vector space. \cite{bolukbasi2016man, garg2018word} demonstrated that these embeddings reflect societal biases. There are also methods to show how these embeddings can be unbiased by aligning them with a set of neutral reference vectors \citep{zhao2018gender, zhao2018learning, caliskan2017semantics, bolukbasi2016man, zhao2019gender}.  These de-biasing methods have however strong limitations, as explained in \citep{gonen2019lipstick}, where the authors show that although the de-biasing embedding methods can reduce the visibility of gender bias, they do not completely eliminate it.

However, there are limitations to \textit{pre-processing} methods. According to \cite{Shah2019Predictive} and \cite{Sun2019Mitigating}, these techniques are limited in detecting and neutralizing all types of bias, especially those deeply ingrained in language or context. The challenge lies in the complexity of biases, which are often subtle and contextually embedded in data.  %{\color {magenta} say a bit about obvious forms of gender bias and less obvious ones.}
Gender biases are linked to gender detection (and therefore to its use by the model). Obvious forms of detection are linked to keywords or expressions used more by one gender than the other. It's these patterns that are detected and corrected by \textit{pre-processing} techniques. 
But language is more complex than that, and sentence construction, syntax and semantics can vary subtly from one genre to another. The most complete models are capable of understanding these subtleties, and we need to build more complex debiasing methods to understand them too. 



%in-processing methods
\paragraph{In-processing methods} A second approach to mitigate biases in AI is to use fairness-aware algorithms, which are specifically designed to take into account the potential for bias and to learn from the data in a way that reduces the risk of making biased decisions.  These are the \emph{in-processing} methods, which generally do not depend on the type of data input.  The advantages of in-processing methods are significant: They actively work to reduce bias during the training phase and are dynamic, adjusting to different forms of bias as the model learns \citep{lu2020gender}.

%{\color {magenta} something like an intro sentence outlining the different methods, adversial, regularization...}
To achieve this, we explore diverse strategies such as adversarial learning, regularization, and fairness metric constraints, each offering a unique approach to mitigating bias.
%adversarial techniques
We can use adversarial Learning by adjusting the discriminator. Adversarial learning involves training a model to make predictions while also training a second model to identify and correct any biases in the first model's predictions. By incorporating this technique into the training process, \cite{zhang2018mitigating, madras2018learning} demonstrate that it is possible to reduce the amount of bias present in machine learning models. 
%Regularization:
Also, a variety of regularization techniques are employed to constrain predictions in the realm of fairness in machine learning. One such method involves using gradient descent to optimize a conventional fairness metric, as discussed in \citep{chuang2021fair}. Beyond this classic approach, there exists a spectrum of regularization strategies aimed at reducing bias. For instance, one can minimize the mutual information between the model's output and the sensitive variable, a technique primarily applied in logistic regression classifiers \citep{kamishima2012fairness}. In a similar vein, the minimization of the Hilbert-Schmidt Independence Criterion (HSIC) between prediction accuracy and sensitive attributes has been proposed by \cite{perez2017fair, li2019kernel}. Furthermore, the application of optimal transport theory to minimize the Wasserstein-2 distance presents an innovative regularization approach for enhancing fairness in predictive models \citep{risser2022tackling}.
%On the other hand, \cite{manisha2018fnnc} mitigate fairness specifically in neural networks.
%constraints
Finally, \cite{zafar2017fairness, zafar2017fairness2} use fairness metrics constraints and solve the training problem subject to those constraints.
All these \textit{in-processing} methods apply in the case of binary classification. There is indeed an \textit{in-processing} paper that proposes a method for multiclass classification for a computer vision task \citep{zhao2017men}, but this paper focuses on the regularization of the mean bias amplification and therefore does not deal with the classic fairness metrics.


However, the main limitations of these methods are that these algorithms can be complex to implement and may sometimes introduce new biases unintentionally. The complexity arises from the sophisticated nature of the algorithms and the need for careful calibration to ensure they do not inadvertently create new forms of bias \citep{Lohia2018Bias}.

%post-processing
\paragraph{Post-processing methods} The last approach is to use \emph{post-processing} de-biasing methods. These methods are model-agnostic and therefore not specific to NLP since they modify the results of previously trained classifiers in order to achieve fairer results.  These methods are applied after a model has been trained, allowing them to adjust outputs to enhance fairness. This adaptability makes them suitable for use on any pre-trained model, providing a versatile tool in the pursuit of reducing bias in AI systems \citep{Lohia2018Bias}.

In this branch, different types of techniques emerged. \cite{menon2018cost} advanced a plugin methodology for the thresholding of predictions, wherein the determination of appropriate thresholds is facilitated through the estimation of class probabilities via logistic regression. Concurrently, \cite{fish2016confidence} developed a confidence-based paradigm, endorsing the assignment of a positive label to each prediction that surpasses a specified threshold, a technique subsequently integrated into AdaBoost \citep{fish2015fair}. This approach diverges from the conventional practice of employing a uniform threshold across all instances, advocating instead for the utilization of group-dependent thresholds, as evidenced in the literature \citep{chzhen2019leveraging, iosifidis2019fae} and presented at the survey \citep{hort2022bia}
In a related vein, \cite{kamiran2012decision, kamiran2018exploiting} introduced the concept of a 'reject option', a novel mechanism that alters the predictions for individuals situated proximate to the decision boundary. This approach is particularly noteworthy for its differential treatment of individuals based on group affiliation, whereby those from unprivileged groups are accorded a positive outcome, in contrast to their privileged counterparts who receive an unfavorable outcome. \cite{chiappa2019path} further enrich this landscape by examining causal models through a counterfactual lens. This approach seeks to align model predictions with a hypothetical scenario where individuals belong to different demographic groups, thus ensuring that the influence of protected attributes is appropriately corrected.

The exploration of \textit{post-processing} methods extends to various contexts, including binary classification \citep{hardt2016equality, sikdar2022getfair} and multiclass classification \citep{denis2021fairness}. While these methods are adept at making outputs fairer, it's important to remember that they tend to address the symptoms rather than the root causes of bias. This means that while they can adjust outputs to be more equitable, they may not eliminate the underlying biases in the training data or the model itself \citep{biswas2020machine}.


\subsection{From Fairness to Explainability}


Ensuring fairness is not solely about neutralizing biases in the data or the model; it is also about understanding and communicating how the algorithm reaches its decisions. This is where the role of explainability comes into play.  %{\color {magenta} right, but something like this has to go up at the beginning of the chapter motivating this jump to explainability}

Explainability, or the ability to elucidate the decision-making process of a machine learning model, stands at the confluence of trustworthiness and transparency. It is the bridge that links the abstract world of algorithmic calculations to the tangible concerns of human users and stakeholders. Without explainability, it becomes challenging to scrutinize or contest a model's decisions, let alone discern whether it is operating fairly or perpetuating harmful stereotypes.

Furthermore, as ML models, especially those in NLP, become more sophisticated and intricate, the opacity of their inner workings intensifies. The "black box" nature of these algorithms not only hampers our ability to identify and rectify biases but also hinders the acceptance and broader adoption of such technologies in critical sectors. To establish trust and ensure the ethical deployment of ML models, it is indispensable to have mechanisms that can elucidate their operations.




\section{Explainability (old)}
The goal of explainability is to make the outputs of these models comprehensible to humans. %Crucially, explainability encompasses various methodologies, including abductive and deductive reasoning for logic, as well as counterfactual explanations. 
Explainability encompasses a variety of methodologies. Within the framework of logical explicability, which pioneered the field, we find deductive and abductive reasoning. Then came counterfactual explanations, and their approximate variants, and contrastive explanations. 

%Abductive reasoning involves forming hypotheses that could explain the observed data {\color {magenta} but they figure as premises in a deductively valid explanation, so abductive explanations are a sort of deductive explanation.  The deductive nomological method comes from Hempel in the 50s.}, while deductive reasoning entails deriving conclusions from known information. {\color  {magenta} this contrast is not right.  Deductively valid explanations are proofs that are logically sound.  That is, the thing to be explained is a logical consequence of the premises or {\em explanans}.  At least abductive explanations like Joao's are also deductively valid explanations, but there is in addition a method to choosing the premises or explanans}. In the context of explainability, abductive reasoning might involve generating hypotheses about why a model made a particular decision, whereas deductive reasoning would apply established rules to understand the decision-making process. 

Deductively valid explanations are essentially proofs characterized by logical soundness. This means that the phenomenon to be explained (the explanandum) is a logical consequence of the premises, or the explanans. This concept of the deductive-nomological method was introduced by Hempel in the 1950s. Abductive explanations can be regarded as a type of deductive explanation with more constraints. Abductive explanations are not only deductively valid but also involve a specific methodology for selecting the premises or explanans. This methodology can vary and is chosen by the creator of the explanations to match their constraints. 
This type of reasoning is mainly used by formal explicability methods \citep{ignatiev2019abduction, marques2023logic}. It provides a solid foundation of rigor, owing to its logical basis. However, in the case of modern models studied in NLP, such as Transformers, which have ever more parameters, these methods show their limits and will therefore not be relevant in the context of this thesis. Consequently, a compromise is necessary, opting for approaches that, while offering fewer guarantees, are more suited to the models in question.


Counterfactual explanations, on the other hand, focus on how altering the input data could change the output. Counterfactual explanations use a different logic from ordinary deductive explanations, which just use typically first order logic or some fragment thereof.  But they can provide valid proofs as well.   These explanations are particularly valuable in understanding complex models, as they provide insights into how different inputs could lead to different predictions or classifications. 
In the same vein, contrastive explanations provide clarity on why a particular event happened as opposed to a different one. These types of explanations are inherently intuitive for humans to both generate and understand. This type of explanation can be found in both formal \citep{ignatiev2020contrastive} and non-formal \citep{jacovi:etal:2021, yin:neubig:2022} methods. 


Moreover, the concepts of faithfulness and plausibility are central to the discussion of explainability. Faithfulness refers to how accurately an explanation reflects the true reasoning process of the model, while plausibility indicates how believable or understandable these explanations are to humans. An ideal explainable AI system would offer both faithful and plausible explanations.



\subsection{Attribution methods}

The most straightforward approach analyzes how each part of the input influences the model's prediction to create saliency maps. These methods are known as attribution methods. Diverse approaches exist for this purpose, including \textit{black-box} and \textit{white-box} methods. \textit{White-box} methods require access to the model's weights and/or gradients, while \textit{black-box} methods only need the input.

\paragraph{}
The \textit{black-box} approach relies on perturbations, which involve the strategic modification of input data and the observation of resultant changes in the model's predictions. The Local Interpretable Model-agnostic Explanations (LIME) technique \citep{ribeiro2016model}, for instance, employs this approach to approximate the model’s behavior locally with an interpretable model, thereby shedding light on the model's operation in specific instances. 
Similarly, \cite{zeiler2014visualizing} employed a visualization technique known as Deconvolutional Network (DeconvNet) to project feature activations back to the input space, thus enabling the visualization of specific input features that activate certain network features.

\cite{lundberg2017unified} introduced SHapley Additive exPlanations (SHAP), a novel approach that integrates the estimation of Shapley values \citep{shapley1953value} with widely recognized explainability techniques such as LIME \citep{LIME} with KernelSHAP, or DeepLIFT \citep{shrikumar2017learning} with DeepSHAP (also introduced by \cite{lundberg2017unified}). Originating from game theory, Shapley Values were initially devised as a method for equitably allocating rewards among participants who collectively contribute to a specific result. SHAP has been adapted and expanded in various ways, detailled in the survey of \cite{mosca2022shap}. \cite{ghorbani2020neuron} tailored SHAP specifically for elucidating predictions from neural networks. Meanwhile, \cite{messalas2019model} and \cite{chen2018shapley} developed alternative methods to approximate Shapley values, enhancing their efficiency and accuracy. Fundamentally, SHAP serves as a framework for local feature-attribution explanations, assigning scores to input features based on their individual contributions at the instance level. However, other methods based on SHAP diverge in their objectives, offering different types of explanations. These range from global explanations \citep{covert2020understanding}, to counterfactual explanations \citep{singal2019shapley} and even concept-based explanations \citep{yeh2020completeness}.


On the other hand, the more classic \textit{white-box} methods are gradient-based methods, which offer a different perspective. \cite{IntegratedGradients} proposed the Integrated Gradients approach, a technique attributing a neural network's prediction to its input features by integrating gradients with respect to the inputs. This method, particularly useful for deep networks, adheres to principles of Sensitivity and Implementation Invariance, aiming to provide a more comprehensive and theoretically grounded understanding of feature importance. 



However, these approaches have weaknesses. 
\cite{wang2020gradient} highlighted a significant vulnerability of gradient-based methods to adversarial manipulation, where minor, often imperceptible perturbations can dramatically alter the interpretations provided by these methods. Also, \cite{adebayo2018sanity} pointed out the issue of partial input recovery in some interpretability methods. Their research suggested that certain methods, especially those reliant on saliency maps, might not fully capture all influential input features, leading to incomplete or skewed interpretations. Lastly, the question of stability in interpretability methods has been raised by \cite{ghorbani2019interpretation}. They demonstrated that minor variations in input, which do not significantly change the model's output, could lead to drastically different interpretations. This lack of stability raises concerns about the consistency and trustworthiness of the interpretations derived from these methods.


It is also possible to create contrastive explanations using attribution methods. The technique is similar, but the paradigm changes. This was achieved by \cite{jacovi:etal:2021, yin:neubig:2022}.


\subsection{Concept-based explanations}

Concept-based explainability is a growing area of research in AI, focused on generating human-understandable explanations for the decisions made by machine learning models. 

\subsubsection{Concept-based XAI for Computer Vision}
The pioneer method TCAV~\citep{kim2018interpretability} goes beyond widespread attribution methods to create high-level explanations based on hand-picked concepts. It uses gradient-based techniques to identify the important features of a model. However, TCAV relies on Human inputs, as it requires the user to manually specify the concepts to be tested. This can be time-consuming and may not always produce the most comprehensive explanations \citep{ghorbani2019towards}.  

Another approach, ACE~\citep{ghorbani2019towards}, aims to automate the concept extraction process. ACE uses a clustering algorithm to identify interpretable concepts in the model's activations, without the need for Human input. While this approach has the potential to greatly reduce the time and effort required for concepts extraction, the authors criticize their own reliance on pre-defined clustering algorithms, which may not always produce the most relevant or useful concepts.

An alternative uses matrix factorization techniques, such as non-negative matrix factorization (NMF)~\citep{lee1999learning}, to identify interpretable factors in the data~\citep{zhang2021invertible,fel:etal:2023}. \cite{fel:etal:2023}  
created a method to discover automatically pertinent concepts inside the network's activation space with NMF and to find the parts of the input space that most align with each concept with Sobol Indices \citep{sobol1993sensitivity}. They successfully tested the meaningfulness and the capacity of these explanations to help Humans understand the model's behavior through psychological experiments. Then, \cite{fel2023holistic} developed a framework for generating global and local explanations to unify automatic concept extraction and concept importance estimation techniques.

However, these approachs have only been applied to convolutional neural networks for image classification tasks so far. The only similar approach to be found in the literature that is totally model agnostic and also applied to textual data is \textit{Concept}SHAP \citep{yeh2020completeness}, a variation of SHAP \citep{lundberg2017unified} that discovers concepts.



\subsubsection{Explaining through rationalization}

For NLP applications, the techniques closest to those based on concepts are those in rationalization. These involve creating a self-interpretable neural architecture capable of simultaneously generating a prediction on classification tasks and its concept-based explanation. 


Researchers in the field of rationalization have proposed specific architectures to extract excerpts from whole inputs and predict a model's output based on these \emph{rationales}~\citep{lei2016rationalizing,jain2020learning,chang2020invariant,yu2019rethinking,bastings2019interpretable,paranjape2020information}. These rationales can be seen as explanations that are sufficiently high-level to be easily understood by humans. 

Finding rationales in text refers to the process of identifying expressions that provide the key reasons or justifications that are provided for a particular claim or decision about that text.  
\citet{lei2016rationalizing} defined rationales as "a minimal set of text spans that are sufficient to support a given claim or decision". They should satisfy two desiderata: they should be interpretable, and they should reach nearly the same prediction as the original output. To do so, they use a generator network that finds interesting excerpts and an encoder network that generates predictions based on them.  However, their scheme requires the use of reinforcement learning~\citep{reinforce} for the optimization procedure. \citet{bastings2019interpretable} proposed to include a reparametrization trick to allow for better gradient estimations without the need for reinforcement learning techniques, and a sparsity constraint to encourage the retrieval of minimal excerpts.

\citet{yu2019rethinking} and \citet{paranjape2020information} studied the problem of producing adequate rationales from a game-theoretic point of view.  However, these models can be quite complex to train, as they either require a reparametrization trick or a reinforcement learning procedure. \citet{jain2020learning} proposed to solve this problem by introducing a support model capable of producing continuous importance scores for instances of the input text, that the rationale extractor can  use to decide whether an excerpt will make  a good rationale or not.

All these rationales will serve as an explanation for single instances, but won't explain how models predict whole classes. \citet{chang2019game} introduced a rationalization technique that allows for the retrieval of rationales for factual and counterfactual scenarios using three players. 



\citet{bouchacourt2019educe} learned concepts without supervision from excerpts using a bidirectional LSTM during the training phase of the model, and the predictions are only based on the presence or absence of the individual concepts in the input sentences.  Going further, \citet{antognini-faltings-2021-rationalization} introduced ConRAT, a technique that includes orthogonality, cosine similarity and knowledge distillation constraints, as well as a concept pruning procedure to improve on both the quality of the extracted concepts and the model's accuracy.


However, rationalization techniques require to train an entirely new model. Only one rationale can also be found per input text, when  there might intuitively be several predictions for a given prediction. Finally, these approaches are not model agnostic and use architectures that have mostly been left behind since the introduction of the Transformer architectures, due to their inferior predictive capabilities.




\subsection{Other methods}
In this section, we address the final group of XAI methods that have not yet been discussed in this thesis, aiming to achieve the most exhaustive state-of-the-art overview possible.

Among these, example-based explainability stands out, utilizing sample-based techniques for generating explanations. This means the explanation’s format is a data point (an example) \citep{poche2023natural}.
The first type, factuals \citep{aamodt1994case}, are similar examples close to the query, helping to understand or justify the model's predictions. For broader insights, counterfactuals and semi-factuals are used. Counterfactuals \citep{wachter2017counterfactual} are the nearest samples with different predictions, while semi-factuals \citep{aryal2023even} are the farthest with similar predictions, both offering a view of the decision boundary. However, to understand how training data alterations might change the model's decisions, influential instances \citep{koh2017understanding} are examined. These are training samples that significantly impact the model's behavior. This approach falls under the umbrella of global explanations. Also falling into this category are Prototypes \citep{molnar2020interpretable}, comprising a selection of samples that represent either the entire dataset or specific classes within it. Typically chosen independently of the model, Prototypes offer an overview of the dataset. However, certain models are crafted with the aid of prototypes and thus can be inherently explained through their design.

Another research path specific for Transformers models harnesses the information in the attention maps of the Transformers' layers to understand how the elements in the input relate to the output, implying that the attention mechanism is inherently interpretable. In spite of a number of supporters initially for this approach, there has been a recent wave of detractors of attention-based explanations~\citep{jain2019attention,pruthi2019learning,serrano2019attention}.

\section{Explainability for Fairness: information removal}

One way of improving the fairness of a model is to employ an approach widespread in information theory, which consists of eliminating information linked to sensitive variables to prevent the model from using them \citep{kilbertus2017avoiding}. This approach to fairness, which we'll call "\textit{sensitive variable information erasure}", has already been examined in various forms in the literature.

A first approach in the literature is to remove explicit gender indicators (\textit{he}, \textit{she}, \textit{her}, etc.) directly from the dataset~\citep{de2019bias}. However, modern Transformer models have been shown to be able to learn implicit gender indicators~\citep{devlin2018bert,karita2019comparative}. This essentially limits the impact that such a naive approach can have on this kind of models. As a matter of fact, a RoBERTa model trained without these gender indicators can still predict with upwards of 90\% accuracy the gender of a person writing a short LinkedIn bio (see Appendix~\ref{apx:genderpredrob}).

Another approach attempts to create word embeddings that do not exhibit gender bias~\citep{bolukbasi2016man, garg2018word, zhao2018gender, zhao2018learning, caliskan2017semantics,bolukbasi2016man,zhao2019gender}. Although interesting in principle, \citet{gonen2019lipstick} shows these methods may camouflage gender biases in word embeddings, but fail to eliminate them entirely. 

A third approach, and more in line with our proposed method, consists in intervening in the model's latent space. In~\citep{liang2020towards}, the authors introduce a technique based on decomposing the latent space using a PCA and subtracting from the inputs the projection into a bias subspace that carries the most information about the target concept. Another vein focuses on modifying the latent space with considerations coming from the field of information theory~\citep{Xu2020A}. Indeed, the $\nu$-information -- a generalization of the mutual information -- has been used as a means to carefully remove from the model's latent space only the information related to the target concept. In particular, popular approaches include the removal of information through linear adversarials on the last layer of the model~\citep{ravfogel2020null,RLACE}, through Assignment-Maximization adversarials~\citep{shao2023erasure}, and through linear models that act on the whole model~\citep{belrose2023leace}. However,  \citet{ravfogel2023loglinear} recently discovered a limitation of guarding with log-linear models on multi-class tasks and warn about the choice of the model used for guarding against the target concept -- \textit{e.g.} the sensitive variable. Clother than this, \cite{frye2020asymmetric,dorleon2022,galhotra2022} use methodology from the field of explainable AI (XAI) to perform feature selection to reduce the effect of algorithmic bias in a human-understandable yet principled manner. 


==> transformermodels.tex <==
\subsection{Transformer models in details}
\begin{figure*}[!htb] 
    \centering
\includegraphics[width=1\linewidth]{images/preliminaries/transformers_architecture.png}
    \caption{Transformer architecture. Figure from \citep{vaswani2017attention}.}
    \label{preliminaries:fig:transformer}
\end{figure*}

\cite{vaswani2017attention} define the transformer by an encoder and a decoder. This general architecture is defined in Figure \ref{preliminaries:fig:transformer}.

In the literature, we also call transformer sub-models of this, with only encoder part or only decoder part. For example, BERT model \citep{devlin2018bert} is a transformer with only encoder part. We focus on this type of transformers in the following.

% \begin{figure}
% \centering
% \begin{tikzpicture}[node distance=2cm]

% % Node styles
% \tikzstyle{mainblock} = [rectangle, draw, minimum width=3cm, minimum height=1cm];
% \tikzstyle{feedforward} = [rectangle, draw, fill=blue!30, minimum width=1.5cm, minimum height=1cm];

% % Nodes
% \node[mainblock, fill=green!30] (attention) {1. Attention};
% \node[above=0.5cm of attention.north west, anchor=south] (z1label) {$Z_1^{k}$};
% \node[above=0.5cm of attention.north east, anchor=south] (z2label) {$Z_2^{k}$};
% \node[mainblock, fill=yellow!30, above=2cm of attention] (addnorm1) {2. Add \& Normalize};
% \node[feedforward, left=4.5cm of addnorm1.north, anchor=south] (ff1) {3. Feed Forward};
% \node[feedforward, right=4.5cm of addnorm1.north, anchor=south] (ff2) {3. Feed Forward};
% \node[mainblock, fill=yellow!30, above=2.5cm of addnorm1] (addnorm2) {4. Add \& Normalize};
% \node[below=0.5cm of addnorm2.south west, anchor=north] (t1label) {$T_1^{k}$};
% \node[below=0.5cm of addnorm2.south east, anchor=north] (t2label) {$T_2^{k}$};

% % Arrows
% \draw[->] (attention.north west) -- (z1label);
% \draw[->] (attention.north east) -- (z2label);
% \draw[->] (z1label) -- (addnorm1.south west);
% \draw[->] (z2label) -- (addnorm1.south east);
% \draw[->] (addnorm1.north west) -- (ff1);
% \draw[->] (addnorm1.north east) -- (ff2);
% \draw[->] (ff1) -- (t1label);
% \draw[->] (ff2) -- (t2label);
% \draw[->] (t1label) -- (addnorm2.south west);
% \draw[->] (t2label) -- (addnorm2.south east);

% % Arrows pointing to Attention block
% \draw[->] ([yshift=-1cm] attention.south west) -- (attention.south west);
% \draw[->] ([yshift=-1cm] attention.south east) -- (attention.south east);
% \node[below=1.1cm of attention.south west] {$T_1^{k-1}$};
% \node[below=1.1cm of attention.south east] {$T_2^{k-1}$};

% % Additional arrows pointing upwards from Add & Normalize block (bloc 4)
% \draw[->] ([xshift=-0.75cm] addnorm2.north) -- ++(0,1cm);
% \draw[->] ([xshift=0 .75cm] addnorm2.north) -- ++(0,1cm);

% \end{tikzpicture}
% \caption{The transformer encoder architecture.}
% \end{figure}


When we have the matrix $X$, we can give it as input to encoder. The encoder is composed of a stack of $N$ identical layers. Each layer has two
sub-layers: \begin{enumerate}
    \item a multi-head self-attention mechanism,
    \item a position-wise fully connected feed-forward network.
\end{enumerate}

Each sub-layer is followed by layer normalization. I.e. the output of sub-layer is LayerNorm(x + Sublayer(x)), where Sublayer(x) is the function implemented by the sub-layer itself.

At the end of the last layer, we have $T^N$ matrix with final embedding for each word of the sentence. 

\subsubsection{Attention mechanism}
We have $W_Q \in \mathbb{R}^{d \times dr}, W_K \in \mathbb{R}^{d \times dr}, W_V \in \mathbb{R}^{d \times dr}$ the weight of Query, Key and Values. In a neural network setting, these weights are usually small numbers, initialised randomly using an appropriate random distribution like Gaussian, Xavier and Kaiming distributions. This initialisation is done once before training.

We note:
\begin{align*}
    Q &= XW_Q \in \mathbb{R}^{ds \times dr} \\
    K &= XW_K \in \mathbb{R}^{ds \times dr} \\
    V &= XW_V \in \mathbb{R}^{ds \times dr}
\end{align*}

%We can also write, for each $x_i$ with $i$ in $1,...,ds$, \begin{align*} Q_i &= x_iW_Q \in \mathbb{R}^{dr} \\
   % K_i &= x_iW_K \in \mathbb{R}^{dr} \\
   % V_i &= x_iW_V \in \mathbb{R}^{dr} \end{align*}

\paragraph{Scaled Dot-Product Attention}
In \textit{Attention is all you need} \cite{vaswani2017attention} we have \textit{Scaled Dot-Product Attention}:

\begin{equation}
    Attention(Q, K, V ) = softmax(\frac{QK^T}{\sqrt{d_k}})V
\end{equation}

This equation use the $softmax$ for matrix. In practice, that means we do, for each $i$ in $1,...,ds$:

\begin{equation*}
    (SC_{i1},...,SC_{ids}) =  softmax(\frac{Q_i K^T}{\sqrt{d_k}}) \in \mathbb{R}^{ds}
\end{equation*}

Softmax is used to create "weights" $SC_{ij}$ with $i,j$ in $1,...,ds$ representing importance of word $X_j$ for word $X_i$. 

\subsubsection{Multi-Head Attention}

We can extend the dot-product attention with multi-head attention. 
Instead of running a single attention function we linearly project the queries, keys and values $H = 8$ times with different learned linear projections on the dimensions $d_q, d_k, d_v$, respectively.
So, we have $H = 8$ outputs $Z_h$ (with $h = 0,...,7$), one for each head. We concatenate the 8 outputs and we multiply with the weight matrix $W^0$ that was trained jointly with the model. The result is the $Z$ matrix that captures information from all attention heads. It has the same shape of the $Z$ matrix learned with the attention model from the previous part.

\subsubsection{Feed Forwards network}
The second sub-layer of each layer in our encoder is a fully connected feed-forward network, which is applied to each position separately and identically. 

These are often two linear transformations with ReLU activation (i.e. $f(z) = max(0,z)$) in between (it's also possible to see different variants as with a GeLU): 
\begin{equation}
    FFN(z) = max(0, zW_1 + b_1 )W_2 + b_2 
\end{equation}

